Path and trajectory planning of a tethered UAV-UGV marsupial robotic system

This letter addresses the problem of trajectory planning in a marsupial robotic system consisting of an unmanned aerial vehicle (UAV) linked to an unmanned ground vehicle (UGV) through a non-taut tether with controllable length. To the best of our knowledge, this is the first method that addresses the trajectory planning of a marsupial UGV-UAV with a non-taut tether. The objective is to determine a synchronized collision-free trajectory for the three marsupial system agents: UAV, UGV, and tether. First, we present a path planning solution based on optimal Rapidly-exploring Random Trees (RRT*) with novel sampling and steering techniques to speed-up the computation. This algorithm is able to obtain collision-free paths for the UAV and the UGV, taking into account the 3D environment and the tether. Then, the letter presents a trajectory planner based on non-linear least squares. The optimizer takes into account aspects not considered in the path planning, like temporal constraints of the motion imposed by limits on the velocities and accelerations of the robots, or raising the tether's clearance. Simulated and field test results demonstrate that the approach generates obstacle-free, smooth, and feasible trajectories for the marsupial system.

==> 04_Results06_B_means_values.tex <==
\begin{table*}[t!]
\caption{B. Statistical analysis for trajectory tracking - From means values (time, vel, acc)}
\centering
\label{tab:realexperiments2_B}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
              & \multicolumn{4}{c|}{UGV} & \multicolumn{5}{c|}{UAV}             & \multicolumn{1}{c|}{Tether}   \\
\hline              
Measure    & Position XY & Time   & Vel.   &   Acc.  & Position XY & Position Z & Time   & Vel    &   Acc.  & 
Length \\
\hline  
Mean error & 0.0337    & 0.4268 & 0.1624 & 0.0751  &
0.0361     & 0.0471    & 1.5768 & 0.1949 & 0.0468  &
0.0001 \\
Max error  & 0.1704    & 2.0664 & 0.8788 & 0.5322 &
0.2370     & 0.3130    & 2.8072 & 0.5610 & 0.2133 &
0.2972 \\
Min error  & 0.0013    & 0.0717 & 0       &  0     &
4.1e-6     & 59.4e-6   & 0.5516 & 0.0448  & 0.0002 &
0 \\    
\hline
\end{tabular}
\end{adjustbox}
\end{table*}




==> 04_Results_03.tex <==
\begin{table*}[t!]
\caption{Results for time execute in the main process inside RRT* algorithm. The term "rand" depicts the time to execute $rand\ node$ process, while "nearest" represents the time to execute $nearest\ node$ process.  The time in $steering\ node$ process is represented by the "steer" term, the time to execute $near\ node$ process by "near" term, and the time to execute connect $process$ and $rewire$ process by "connect" and "rewire", respectively.}
\centering
\label{tab:experiments3}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c}{\begin{tabular}[c]{@{}c@{}}SI \end{tabular}} &
\multicolumn{1}{|c}{\begin{tabular}[c]{@{}c@{}}rand [$\mu$s]\end{tabular}} & \multicolumn{1}{|c}{\begin{tabular}[c]{@{}c@{}}nearest[$\mu$s]\end{tabular}} & 
\multicolumn{1}{|c}{\begin{tabular}[c]{@{}c@{}}steer [$m$s]\end{tabular}} & \multicolumn{1}{|c}{\begin{tabular}[c]{@{}c@{}}near [$m$s]\end{tabular}} & \multicolumn{1}{|c}{\begin{tabular}[c]{@{}c@{}}connect [$m$s]\end{tabular}} &
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}rewire [$m$s]\end{tabular}} \\
\hhline{|=|=|=|=|=|=|=|}
S4.1 & 26.37 & 364.9  & 23.60 & 6.121 & 9.652  & 3.377 \\
S5.1 & 42.02 & 954.7  & 41.51 & 24.82 & 30.02  & 10.40 \\

\hline
\end{tabular}
\end{adjustbox}
\vspace*{-2mm}
\end{table*}

%\begin{table*}[ht]
%\caption{Results for compute time for RRT* algorithm. "last sol" is the timed that was found solution with minimum cost. "total iter" is the algorithm time to execute 20.000 iterations.}
%\centering
%\label{tab:experiments4}
%\begin{adjustbox}{max width=\textwidth}
%\begin{tabular}{|l|l|l|}
%\hline
%\multicolumn{1}{|c}{\begin{tabular}[c]{@{}c@{}}SI\end{tabular}} &
%\multicolumn{1}{|c}{\begin{tabular}[c]{@{}c@{}}last sol\end{tabular}} &
%\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}total iter\end{tabular}} \\
%\hhline{|=|=|=|}
%S4.1  &  32.8  &  455.2      \\
%s5.1  &  47.5  &  1143.4     \\    

%\hline
%\end{tabular}
%\end{adjustbox}
%\vspace*{-2mm}
%\end{table*}

==> 04_Results_04.tex <==
\begin{table*}[t!]
\caption{Experiments results for compute UAV position, real UAV position, compute length and real length}
\centering
\label{tab:experiments}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lll|lll|lll|ll|l}
\hline

Compute X & Compute Y & Compute Z & Real X  & Real Y  & Real Z & Error X & Error Y & Error Z & Compute L & Real L  & Error L \\
\hhline{|=|=|=|=|=|=|=|=|=|=|=|=}
53.0000   & 11.0000   & 4.8000    & 53.8222 & 11.7889 & 5.0332 & -0.0155 & -0.0717 & -0.0486 & 6.7000    & 6.6762  & 0.0036  \\
52.8571   & 11.0714   & 4.8714    & 52.9399 & 10.9877 & 4.7986 & -0.0016 & 0.0076  & 0.0150  & 6.7857    & 6.7564  & 0.0043  \\
52.7143   & 11.1429   & 4.9429    & 52.9427 & 10.9110 & 4.8048 & -0.0043 & 0.0208  & 0.0279  & 6.8714    & 6.8459  & 0.0037  \\
52.5714   & 11.2143   & 5.0143    & 52.8385 & 11.1522 & 5.0413 & -0.0051 & 0.0055  & -0.0054 & 6.9571    & 6.9322  & 0.0036  \\
52.4286   & 11.2857   & 5.0857    & 52.5713 & 11.2397 & 4.9037 & -0.0027 & 0.0041  & 0.0358  & 7.0429    & 7.0155  & 0.0039  \\
52.2857   & 11.3571   & 5.1571    & 52.5926 & 11.2601 & 4.9432 & -0.0059 & 0.0085  & 0.0415  & 7.1286    & 7.1049  & 0.0033  \\
52.1429   & 11.4286   & 5.2286    & 52.3652 & 11.1319 & 5.1141 & -0.0043 & 0.0260  & 0.0219  & 7.2143    & 7.1836  & 0.0043  \\
52.0000   & 11.5000   & 5.3000    & 52.1744 & 11.1852 & 5.2593 & -0.0034 & 0.0274  & 0.0077  & 7.3000    & 7.2592  & 0.0056  \\
51.8571   & 11.5714   & 5.3714    & 51.9868 & 10.9174 & 5.5045 & -0.0025 & 0.0565  & -0.0248 & 7.4000    & 7.3640  & 0.0049  \\
51.7143   & 11.6429   & 5.4429    & 51.9683 & 11.9109 & 5.3243 & -0.0049 & -0.0230 & 0.0218  & 7.5000    & 7.4799  & 0.0027  \\
51.5714   & 11.7143   & 5.5143    & 51.7378 & 11.5771 & 5.4235 & -0.0032 & 0.0117  & 0.0165  & 7.6000    & 7.5747  & 0.0033  \\
51.4286   & 11.7857   & 5.5857    & 51.8172 & 11.5055 & 5.4151 & -0.0076 & 0.0238  & 0.0306  & 7.7000    & 7.6745  & 0.0033  \\
51.2857   & 11.8571   & 5.6571    & 51.3412 & 11.8806 & 5.5995 & -0.0011 & -0.0020 & 0.0102  & 7.8000    & 7.7736  & 0.0034  \\
51.1429   & 11.9286   & 5.7286    & 51.4606 & 11.8551 & 5.5808 & -0.0062 & 0.0062  & 0.0258  & 7.9000    & 7.8749  & 0.0032  \\
51.0000   & 12.0000   & 5.8000    & 51.3415 & 11.8818 & 5.7318 & -0.0067 & 0.0098  & 0.0118  & 8.0000    & 7.9705  & 0.0037  \\
50.8571   & 12.0714   & 5.8714    & 51.0855 & 12.1975 & 5.7798 & -0.0045 & -0.0104 & 0.0156  & 8.1714    & 8.1324  & 0.0048  \\
50.7143   & 12.1429   & 5.9429    & 50.8958 & 12.1582 & 5.8301 & -0.0036 & -0.0013 & 0.0190  & 8.3429    & 8.3109  & 0.0038  \\
50.5714   & 12.2143   & 6.0143    & 50.8983 & 12.1735 & 5.8504 & -0.0065 & 0.0033  & 0.0273  & 8.5143    & 8.4855  & 0.0034  \\
50.4286   & 12.2857   & 6.0857    & 50.6360 & 12.1996 & 6.0279 & -0.0041 & 0.0070  & 0.0095  & 8.6857    & 8.6540  & 0.0036  \\
50.2857   & 12.3571   & 6.1571    & 50.6782 & 12.2602 & 6.0087 & -0.0078 & 0.0078  & 0.0241  & 8.8571    & 8.8344  & 0.0026  \\
50.1429   & 12.4286   & 6.2286    & 50.3307 & 12.5545 & 6.3111 & -0.0037 & -0.0101 & -0.0133 & 9.0286    & 9.0041  & 0.0027  \\
50.0000   & 12.5000   & 6.3000    & 50.3664 & 12.5167 & 6.1394 & -0.0073 & -0.0013 & 0.0255  & 9.2000    & 9.1737  & 0.0029  \\
49.8571   & 12.5714   & 6.3714    & 50.0907 & 12.4682 & 6.4354 & -0.0047 & 0.0082  & -0.0100 & 9.3571    & 9.3357  & 0.0023  \\
49.7143   & 12.6429   & 6.4429    & 50.0304 & 12.5023 & 6.3975 & -0.0064 & 0.0111  & 0.0070  & 9.5143    & 9.4766  & 0.0040  \\
49.5714   & 12.7143   & 6.5143    & 49.7741 & 12.6129 & 6.4241 & -0.0041 & 0.0080  & 0.0138  & 9.6714    & 9.6339  & 0.0039  \\
49.4286   & 12.7857   & 6.5857    & 49.6836 & 12.6474 & 6.4875 & -0.0052 & 0.0108  & 0.0149  & 9.8286    & 9.8013  & 0.0028  \\
49.2857   & 12.8571   & 6.6571    & 49.4600 & 12.7895 & 6.5173 & -0.0035 & 0.0053  & 0.0210  & 9.9857    & 9.9583  & 0.0027  \\
49.1429   & 12.9286   & 6.7286    & 49.4252 & 12.8980 & 6.5728 & -0.0057 & 0.0024  & 0.0232  & 10.1429   & 10.1152 & 0.0027  \\
49.0000   & 13.0000   & 6.8000    & 49.2767 & 12.9657 & 6.7452 & -0.0056 & 0.0026  & 0.0081  & 10.3000   & 10.2672 & 0.0032  \\
48.8571   & 13.0714   & 6.8714    & 49.0968 & 12.9984 & 6.8977 & -0.0049 & 0.0056  & -0.0038 & 10.4000   & 10.3801 & 0.0019  \\
48.7143   & 13.1429   & 6.9429    & 49.0155 & 13.1023 & 6.8986 & -0.0062 & 0.0031  & 0.0064  & 10.5000   & 10.4641 & 0.0034  \\
48.5714   & 13.2143   & 7.0143    & 48.7847 & 13.2039 & 6.9737 & -0.0044 & 0.0008  & 0.0058  & 10.6000   & 10.5651 & 0.0033  \\
48.4286   & 13.2857   & 7.0857    & 48.8291 & 13.2906 & 7.0265 & -0.0083 & -0.0004 & 0.0084  & 10.7000   & 10.6695 & 0.0029  \\
48.2857   & 13.3571   & 7.1571    & 48.6507 & 13.1510 & 7.2074 & -0.0076 & 0.0154  & -0.0070 & 10.8000   & 10.7685 & 0.0029  \\
48.1429   & 13.4286   & 7.2286    & 48.4196 & 13.3720 & 7.1049 & -0.0057 & 0.0042  & 0.0171  & 10.9000   & 10.9228 & -0.0021 \\
48.0000   & 13.5000   & 7.3000    & 48.2837 & 13.4116 & 7.1107 & -0.0059 & 0.0065  & 0.0259  & 11.0000   & 11.0326 & -0.0030 \\
\hline
\end{tabular}
\end{adjustbox}
\vspace*{-2mm}
\end{table*}

==> 04_Results_05.tex <==
\begin{table*}[t!]
\caption{Experimental results for computed UAV position, real UAV position, compute length and real length}
\centering
\label{tab:realexperiments1}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{3}{|c}{\begin{tabular}[c]{@{}c@{}}Position UAV \end{tabular}} &
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}Tether \end{tabular}} \\
\hline
Error X [\%] & Error Y [\%] & Error Z [\%] & Error L [\%] \\
\hhline{|=|=|=|=}
0.5294 & 0.5274  & 1.1832  & 0.3093\\
\hline
\end{tabular}
\end{adjustbox}
\vspace*{-2mm}
\end{table*}

